A monolithic approach to fluid-structure interaction based on a hybrid Eulerian-ALE fluid domain decomposition involving cut elements

A novel method for complex fluid-structure interaction (FSI) involving large structural deformation and motion is proposed. The new approach is based on a hybrid fluid formulation that combines the advantages of purely Eulerian (fixed-grid) and Arbitrary-Lagrangian-Eulerian (ALE moving mesh) formulations in the context of FSI. The structure - as commonly given in Lagrangian description - is surrounded by a fine resolved layer of fluid elements based on an ALE-framework. This ALE-fluid patch, which is embedded in an Eulerian background fluid domain, follows the deformation and motion of the structural interface. This approximation technique is not limited to Finite Element Methods, but can can also be realized within other frameworks like Finite Volume or Discontinuous Galerkin Methods. In this work, the surface coupling between the two disjoint fluid subdomains is imposed weakly using a stabilized Nitsche's technique in a Cut Finite Element Method (CutFEM) framework. At the fluid-solid interface, standard weak coupling of node-matching or non-matching finite element approximations can be utilized. As the fluid subdomains can be meshed independently, a sufficient mesh quality in the vicinity of the common fluid-structure interface can be assured. To our knowledge the proposed method is the only method (despite some overlapping domain decomposition approaches that suffer from other issues) that allows for capturing boundary layers and flow detachment via appropriate grids around largely moving and deforming bodies and is able to do this e.g. without the necessity of costly remeshing procedures. In addition it might also help to safe computational costs as now background grids can be much coarser. Various FSI-cases of rising complexity conclude the work.

==> operators.tex <==
%---------------------------------------------------------------------------------------------
\newcommand{\TODO}[1]{\color{red} TODO: #1 \color{black}}

%\definecolor{darkblue}{rgb}{0.27 0.52 0.60}
\newcommand{\figref}[1]{Fig.\,\ref{#1}}
\newcommand{\Eqref}[1]{Eq.\,\eqref{#1}}
\newcommand{\Tabref}[1]{Tab.\,\ref{#1}}
\newcommand{\algref}[1]{Alg.\,\ref{#1}}

%\definecolor{darkblue}{rgb}{0.27 0.52 0.60}

%--------------------------
% Reference systems
\newcommand{\lagr}{\textbf{X}}
\newcommand{\euler}{\textbf{x}}
\newcommand{\ale}{\boldsymbol{\chi}}

\newcommand{\x}{\boldsymbol{x}}

\newcommand{\trans}{\text{T}}

%domains
\newcommand{\domainbf}{\Omega^{b}}
\newcommand{\domainbfvoid}{\Omega^{b-}}
%\newcommand{\domainbfnp}{\Omega^{b,n+1}}
\newcommand{\domainef}{\Omega^{e}}
%\newcommand{\domainefnp}{\Omega^{e,n+1}}
\newcommand{\domaini}{\Omega^{i}}
\newcommand{\interfaceff}{\Gamma^{\text{FF}}}
\newcommand{\interfaceffnp}{\Gamma^{\text{FF}}(t^{n+1})}
\newcommand{\neumannbnp}{\bar{\boldsymbol{h}}^{b,n+1}}
\newcommand{\domains}{\Omega^{s}}
\newcommand{\interfacefsi}{\Gamma^{\text{FSI}}}
\newcommand{\domainf}{\Omega^{\text{f}}}
\newcommand{\domainale}{\Omega^{\text{ALE}}}
\newcommand{\unit}[1]{\mathrm{#1}} % unit
% physicalische Groeßen
%fluid
\newcommand{\density}{\rho^{\text{f}}}
\newcommand{\dynvisc}{\mu}
\newcommand{\kinvisc}{\nu}
\newcommand{\vel}{\boldsymbol{u}}
\newcommand{\veli}{\boldsymbol{u}^{i}}
\newcommand{\velb}{\boldsymbol{u}^{b}}
\newcommand{\vele}{\boldsymbol{u}^{e}}
\newcommand{\velg}{\boldsymbol{u}^{{g}}}
\newcommand{\press}{p}
\newcommand{\pressdyn}{p_{\text{dyn}}}
\newcommand{\pressb}{p^{b}}
\newcommand{\presse}{p^{e}}
\newcommand{\pressi}{p^{i}}
\newcommand{\bodyfb}{\boldsymbol{b}^{b}}
\newcommand{\body}{\boldsymbol{b}}
\newcommand{\bodyfe}{\boldsymbol{b}^{e}}
\newcommand{\bodyfi}{\boldsymbol{b}^{i}}
\newcommand{\konve}{\boldsymbol{c}^{e}} % konvective velocity
\newcommand{\konv}{\boldsymbol{c}} % konvective velocity
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\normalb}{\boldsymbol{n}^{b}}
\newcommand{\normale}{\boldsymbol{n}^{e}}
\newcommand{\normalfi}{\boldsymbol{n}^{F,i}}
\newcommand{\neumannb}{\bar{\boldsymbol{h}}^{b}}
\newcommand{\neumann}{\bar{\boldsymbol{h}}}

%fluid residual based stabilization
\newcommand{\resmomi}{\boldsymbol{r}^{m,i}}
\newcommand{\resmomh}{\boldsymbol{r}_{\euler,h}^m}
\newcommand{\resmomALEh}{\boldsymbol{r}_{\ale,h}^{m}}
\newcommand{\resmomih}{\boldsymbol{r}_{h}^{m,i}}
\newcommand{\resmomb}{\boldsymbol{r}^{m,b}}
\newcommand{\resmombh}{\boldsymbol{r}^{m,b}_h}
\newcommand{\resmomeh}{\boldsymbol{r}^{m,e}_h}
\newcommand{\resmome}{\boldsymbol{r}^{m,e}}
\newcommand{\resconti}{\boldsymbol{r}^{c,i}}
\newcommand{\rescontb}{\boldsymbol{r}^{c,b}}
\newcommand{\rescontbh}{\boldsymbol{r}^{c,b}_h}
\newcommand{\resconte}{\boldsymbol{r}^{c,e}}
\newcommand{\resconteh}{\boldsymbol{r}^{c,e}_h}
\newcommand{\resconth}{\boldsymbol{r}_{h}^c}
\newcommand{\ele}{\text{\small{e}}}
% edgebased and gp
\newcommand{\GP}{\textsc{\tiny{GP}}}
\newcommand{\FOS}{\textsc{\tiny{FOS}}}
\newcommand{\Inf}{\textsc{\tiny{Inf}}}


%fsi Größen fluid
\newcommand{\fsitraction}{{\boldsymbol{h}}^{e}_{\interfacefsi}}
\newcommand{\tlambda}{\delta \boldsymbol{\uplambda}}
\newcommand{\fsilambda}{\boldsymbol{\uplambda}}
\newcommand{\fsilambdah}{\boldsymbol{\uplambda}_h}
\newcommand{\tlambdah}{\delta \boldsymbol{\uplambda}_h}
% ALE groeßen
\newcommand{\embdisp}{\boldsymbol{d}^{{g}}}
\newcommand{\embvelgrid}{\boldsymbol{u}^{{g}}}
\newcommand{\embdisph}{\boldsymbol{d}^{{g}}_h}
\newcommand{\embdispint}{\boldsymbol{d}^{{g}}_{\interfacefsi}}
\newcommand{\embdispnp}{\boldsymbol{d}^{{g},n+1}}
\newcommand{\embdispn}{\boldsymbol{d}^{{g},n}}
\newcommand{\cauchystressale}{\boldsymbol{\sigma}^{g}}
\newcommand{\viscale}{\boldsymbol{\epsilon^{g}}}
\newcommand{\alepoisson}{\nu^{g}}

% structure großen
\newcommand{\strdensity}{\rho^\text{s}}
\newcommand{\disp}{\boldsymbol{d}^s}
\newcommand{\disph}{\boldsymbol{d}^s_h}
 \newcommand{\dispini}{\boldsymbol{d}^{s}_0}
\newcommand{\dispnp}{\boldsymbol{d}^{s,n+1}}
\newcommand{\tdisp}{\delta \boldsymbol{d}^s}
\newcommand{\tdisph}{\delta \boldsymbol{d}^s_h}
\newcommand{\bodyfs}{\boldsymbol{b}^{s}}
\newcommand{\piolak}{\boldsymbol{S}}
\newcommand{\cauchystressstr}{\boldsymbol{\sigma}^s}
\newcommand{\deformationsgrad}{\boldsymbol{F}}
\newcommand{\greenlagr}{\boldsymbol{E}}
\newcommand{\cauchygreen}{\boldsymbol{C}}
\newcommand{\neumanns}{\bar{\boldsymbol{h}}^{s}}
\newcommand{\fsitractionstr}{{\boldsymbol{h}}^{s}_{\interfacefsi}}
\newcommand{\strainenergy}{{{\Psi}}}
\newcommand{\strainenergysvk}{{{\Psi}}_{\textsc{\tiny{SVK}}}}
\newcommand{\strainenergynh}{{{\Psi}}_{\textsc{\tiny{NH}}}}
\newcommand{\strpoisson}{\nu^s}
\newcommand{\strnormal}{\boldsymbol{n}^{s}}
%structure matrix größen
\newcommand{\formfunctions}{\mathsf{N}^\text{s}}
\newcommand{\massenmatrs}{\mathsf{M}^\text{s}}
\newcommand{\internfs}{\mathsf{F}^\text{s}_{\textrm{int}}}
\newcommand{\externfs}{\mathsf{F}^\text{s}_{\textrm{ext}}}
\newcommand{\externfsalphas}{\mathsf{F}^{\text{s},n+1-\alpha_f}_{\textrm{ext}}}
\newcommand{\externfsnps}{\mathsf{F}^{\text{s},n+1}_{\textrm{ext}}}
\newcommand{\externfsns}{\mathsf{F}^{\text{s},n}_{\textrm{ext}}}
\newcommand{\resstr}{\mathsf{F}^{\text{s}}_{\textrm{res}}}
%fluid matrix größen
\newcommand{\massenmatrf}{\mathsf{M}^\text{F}}
\newcommand{\convmatrf}{\mathsf{C}^\text{F}}
\newcommand{\viscmatrf}{\mathsf{K}^\text{F}}
\newcommand{\gmatrf}{\mathsf{G}^\text{F}}
\newcommand{\matrforce}{\mathsf{f}}
\newcommand{\fluidstabmatr}{{\mathsf{\underline{S}}}}
\newcommand{\supgmatr}{\mathsf{S}^\text{SUPG}}
\newcommand{\pspgmatr}{\mathsf{S}^\text{PSPG}}
\newcommand{\bvmatr}{\mathsf{S}^\text{BV}}

%discrete nodal vectors
\newcommand{\dnvelb}{\mathsf{u}^{\text{b}}}
\newcommand{\dnvelbk}{\mathsf{u}^{\text{b},K}}
\newcommand{\dnvelenp}{\mathsf{u}^{\text{e},n+1}}
\newcommand{\dnvelen}{\mathsf{u}^{\text{e},n}}
\newcommand{\dnvele}{\mathsf{u}^{\text{e}}}
\newcommand{\dnvelek}{\mathsf{u}^{\text{e},K}}
\newcommand{\dnvel}{\mathsf{{u}}}
\newcommand{\dnvelall}{\mathsf{{u}}^\text{ff}}
\newcommand{\dnpresall}{\mathsf{{p}}^\text{ff}}
\newcommand{\dnvelnp}{\mathsf{u}^{n+1}}
%%%%%%%%%TODO
%\newcommand{\dnvelinner}{\dnvel_\inner^{b,e}}
\newcommand{\dnvelinnernpip}{\dnvel_{\inner,i+1}^{\text{ff},n+1}}
%\newcommand{\dnvelbound}{\dnvel_\bound^{e}}
%\newcommand{\dnvelboundip}{\dnvel_{\bound,i+1}^{e}}
%\newcommand{\dnvelboundn}{\dnvel_\bound^{e,n}}

\newcommand{\dnpressb}{\mathsf{p}^{\text{b}}}
\newcommand{\dnpressbk}{\mathsf{p}^{\text{b},K}}
\newcommand{\dnpresse}{\mathsf{p}^{\text{e}}}
\newcommand{\dnpressek}{\mathsf{p}^{\text{e},K}}
\newcommand{\dnpress}{\mathsf{p}}
\newcommand{\dnpressnp}{\mathsf{p}^{n+1}}
%structure--------------------------
\newcommand{\dndisps}{\mathsf{d}^{\text{s}}}
\newcommand{\dndispnps}{\mathsf{d}^{\text{s},n+1}}
\newcommand{\dndispalphas}{\mathsf{d}^{\text{s},n+1-\alpha_f}}
\newcommand{\dndispns}{\mathsf{d}^{\text{s},n}}
\newcommand{\dnaccnps}{{\ddot{\mathsf{d}}}^{\text{s},n+1}}
\newcommand{\dnaccalphas}{{\ddot{\mathsf{d}}}^{\text{s},n+1-\alpha_m}}
\newcommand{\dnaccns}{{\ddot{\mathsf{d}}}^{\text{s},n}}
\newcommand{\dnvelns}{{\dot{\mathsf{d}}}^{\text{s},n}}
\newcommand{\dnvelnps}{{\dot{\mathsf{d}}}^{\text{s},n+1}}
\newcommand{\dnvelalphas}{{\dot{\mathsf{d}}}^{\text{s},n+1-\alpha_f}}
\newcommand{\dnembdisp}{\mathsf{d}^{\text{g}}}
\newcommand{\dnembdispnp}{\mathsf{d}^{\text{g},n+1}}
\newcommand{\dnembdispn}{\mathsf{d}^{\text{g},n}}
\newcommand{\dnfsilambda}{\mathsf{\lambda}}
\newcommand{\dnx}{\mathsf{{x}}}
\newcommand{\dnxf}{\mathsf{x}^\text{ff}}
%-------------------------------------------------
\newcommand{\dncauchystress}{\mathsf{\bar\sigma}^{\text{b}}}
\newcommand{\dncauchystressk}{\mathsf{\bar\sigma}^{\text{b},K}}

%Nitsche parameter
\newcommand{\betan}{\beta_{\text{n}}}
%MHVS parameter
\newcommand{\betav}{\beta_{\text{v}}}

%fsi Größen matrix
\newcommand{\fluidres}{\mathsf{r}^\text{f}}
\newcommand{\fluidresall}{\mathsf{r}^\text{ff}}
\newcommand{\fluidresgeneral}{\mathsf{r}}
\newcommand{\fluidresnp}{\mathsf{r}^{\text{ff},n+1}}
\newcommand{\structureres}{\mathsf{r}^\text{s}}
\newcommand{\structureresnp}{\mathsf{r}^\text{s,n+1}}
\newcommand{\gridres}{\mathsf{r}^\text{g}}
\newcommand{\couplingres}{\mathsf{r}^\text{kin}}
\newcommand{\allres}{\mathsf{r}^\text{FSI}}
\newcommand{\fluidresm}{\mathsf{r}^{\text{ff},m}}
\newcommand{\res}{\mathsf{r}}
\newcommand{\structureresm}{\mathsf{r}^{\text{s},m}}

%fixed-ale approach
\newcommand{\dnembdispff}{{\mathsf{d}}^\text{g}_{\interfaceff}}
\newcommand{\dnembdispfsi}{{\mathsf{{d}}}^{\text{g}}_{\interfacefsi}}
\newcommand{\dnvelbdef}{{\mathsf{{u}}}^{\text{b}}_\text{def}}
\newcommand{\dnveldef}{{\mathsf{{u}}}^\text{ff}_\text{def}}
\newcommand{\dnveledef}{{\mathsf{{u}}}^{\text{e}}_\text{def}}
\newcommand{\dnveledeffsi}{{\mathsf{{u}}}^{\text{e}}_{\text{def},\interfacefsi}}
\newcommand{\dndispdef}{{\mathsf{{d}}}^{\text{s}}_\text{def}}
\newcommand{\dnxdef}{\mathsf{x}_\text{def}^{n+1}}
%\newcommand{\dndispnp}{{\textsf{\boldmath{d}}}^{s,n+1}}
\newcommand{\dnembdispdef}{{\mathsf{{d}}}^{\text{g}}_\text{def}}

% Assembly
%\newcommand{\assembly}{\large{\mathbf{A}}}

% \newcommand{\assemblyfont}[1]{\mathrm{#1}}
\newcommand{\assemblyfont}[1]{{#1}}
\newcommand{\assembly}[3][d]{%  % assembly operator
% option 'd' is useless
\mathchoice{  % display style
\overset{#3}{\underset{#2}{\raisebox{-0.6ex}{\mbox{\huge \assemblyfont{A}}}}}
}{  % text style
\raisebox{-0.35ex}{\mbox{\Large \assemblyfont{A}}}_{#2}^{#3}
}{  % script style
\raisebox{-0.35ex}{\mbox{\Large \assemblyfont{A}}}_{#2}^{#3}
}{  % scriptscript style
\raisebox{-0.35ex}{\mbox{\Large \assemblyfont{A}}}_{#2}^{#3}
}}

%matrix FSI
\newcommand{\fluidmatr}{\mathsf{F}}
\newcommand{\fluidmatrst}{\mathsf{Fs}}
\newcommand{\fluidmatrall}{\mathsf{F}^\text{ff}}
\newcommand{\fluidmatrG}{\mathsf{F}^\text{g}}
\newcommand{\strmatr}{\mathsf{S}}
\newcommand{\alematr}{\mathsf{A}}
\newcommand{\csfmatr}{\mathsf{C}_{\text{SF}}}
\newcommand{\cfsmatr}{\mathsf{C}_{\text{FS}}}
\newcommand{\jacobi}{\mathsf{J}}
\newcommand{\inner}{\text{I}}
\newcommand{\bound}{\Gamma}

%%%%%%%%%%%%%%%matrix fluid-fluid%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Residuals
%\newcommand{\fluidresff}[2]{\boldsymbol{r}_{#2^{#1}}}
%\newcommand{\fluidresffstd}[2]{\boldsymbol{r}^{\text{std}}_{#2^{#1}}}

%residuum governing equations fluid
% \newcommand{\fluidresmomstd}{\mathsf{F}^{\text{M,std}}_{\textrm{res}}}
% \newcommand{\fluidrescontstd}{\mathsf{F}^{\text{C,std}}_{\textrm{res}}}
% \newcommand{\fluidresmomstab}{\mathsf{F}^{\text{M,stab}}_{\textrm{res}}}
% \newcommand{\fluidrescontstab}{\mathsf{F}^{\text{C,stab}}_{\textrm{res}}}
% 
% \newcommand{\fluidresmomall}{\mathsf{F}^{\text{M}}_{\textrm{res}}}
% \newcommand{\fluidrescontall}{\mathsf{F}^{\text{C}}_{\textrm{res}}}

%% residuals discrete weak form
\newcommand{\tfluidresff}[2]{R_{#2^{#1}}}
\newcommand{\tfluidresffstd}[2]{R^{\text{std}}_{#2^{#1}}}
\newcommand{\tfluidresfstd}[1]{R^{\text{std}}_{\euler,#1}}
\newcommand{\tfluidresfstdALE}[1]{R^{\text{std}}_{\ale,#1}}
\newcommand{\tfluidresfstab}[1]{R^{\text{stab}}_{#1}}% stabiliziert 
%%%%% matrix
\newcommand{\couplbmatr}{\mathsf{G}}
\newcommand{\coupldmatr}{\mathsf{K}}
\newcommand{\couplcmatr}{\mathsf{C}} %stressbased
\newcommand{\couplbmatrall}{\mathsf{\underline{G}}}
%%%rechteseite
\newcommand{\fluidresstab}{\mathsf{r}^\text{stab}} %stabilisiert
\newcommand{\fluidresb}{\mathsf{r}^\text{b}}
\newcommand{\fluidresbK}{\mathsf{r}^{\text{b},K}}
\newcommand{\fluidrese}{\mathsf{r}^\text{e}}
\newcommand{\fluidreseK}{\mathsf{r}^{\text{e},K}}
\newcommand{\fluidrescb}{\mathsf{c}^\text{b}} %stressbased
\newcommand{\fluidresce}{\mathsf{c}^\text{e}} %stressbased
\newcommand{\fluidrescbK}{\mathsf{c}^{\text{b},K}} %stressbased
\newcommand{\fluidresceK}{\mathsf{c}^{\text{e},K}} %stressbased


%time discrete
\newcommand{\velbhist}{\boldsymbol{u}^{b,\text{hist}}}
\newcommand{\velhist}{\boldsymbol{u}^{\text{hist}}}
\newcommand{\velbhisth}{\boldsymbol{u}^{b,\text{hist}}_h}
\newcommand{\velihisth}{\boldsymbol{u}^{i,\text{hist}}_h}
\newcommand{\velehist}{\boldsymbol{u}^{e,\text{hist}}}
\newcommand{\velehisth}{\boldsymbol{u}^{e,\text{hist}}_h}
\newcommand{\velbn}{\boldsymbol{u}^{b,n}}
\newcommand{\veln}{\boldsymbol{u}^{n}}
\newcommand{\velbnh}{\boldsymbol{u}^{b,n}_h}
\newcommand{\velinh}{\boldsymbol{u}^{i,n}_h}
\newcommand{\velen}{\boldsymbol{u}^{e,n}}
\newcommand{\velenh}{\boldsymbol{u}^{e,n}_h}
\newcommand{\velenp}{\boldsymbol{u}^{e,n+1}}
\newcommand{\velbnguess}{\tilde{\boldsymbol{u}}^{b,n}}
\newcommand{\velenguess}{\tilde{\boldsymbol{u}}^{e,n}}
\newcommand{\velbhisthguess}{\tilde{\boldsymbol{u}}^{b,\text{hist}}_h}
\newcommand{\velbndot}{\dot{\boldsymbol{u}}^{b,n}}
\newcommand{\velndot}{\dot{\boldsymbol{u}}^{n}}
\newcommand{\velbndoth}{\dot{\boldsymbol{u}}^{b,n}_h}
\newcommand{\velendoth}{\dot{\boldsymbol{u}}^{e,n}_h}
\newcommand{\velindoth}{\dot{\boldsymbol{u}}^{i,n}_h}
\newcommand{\velbndotguess}{\tilde{\dot{\boldsymbol{u}}}^{b,n}}
\newcommand{\velbndotguessh}{\tilde{\dot{\boldsymbol{u}}}^{b,n}_h}
\newcommand{\velbnguessh}{\tilde{{\boldsymbol{u}}}^{b,n}_h}
\newcommand{\velendot}{\dot{\boldsymbol{u}}^{e,n}}
\newcommand{\velbnhat}{\tilde{\boldsymbol{u}}^{b,n}}
\newcommand{\abn}{\boldsymbol{a}^{b,n}}
\newcommand{\aen}{\boldsymbol{a}^{e,n}}
\newcommand{\velbnhath}{\tilde{\boldsymbol{u}}^{b,n}_h}
%master-slave vectors 
%\newcommand{\velmh}{\boldsymbol{u}^m_h}
%\newcommand{\velmh}{p^m_h}
%\newcommand{\tvelmh}{\boldsymbol{v}^m_h}
%\newcommand{\tpressmh}{q^{m}_h}

% discrete Groeßen
\newcommand{\velh}{\boldsymbol{u}_h}
\newcommand{\velhnp}{\boldsymbol{u}_h^{n+1}}
\newcommand{\velbh}{\boldsymbol{u}^b_h}
\newcommand{\veleh}{\boldsymbol{u}^e_h}
\newcommand{\pressh}{p_h}
\newcommand{\presshnp}{p_h^{n+1}}
\newcommand{\pressbh}{p^{b}_h}
\newcommand{\presseh}{p^e_h}
\newcommand{\pressih}{p^i_h}
\newcommand{\tvelbh}{\boldsymbol{v}^b_h}
\newcommand{\tveleh}{\boldsymbol{v}^e_h}
\newcommand{\tvelh}{\boldsymbol{v}_{h}}
\newcommand{\tvelih}{\boldsymbol{v}^i_h}
\newcommand{\velih}{\boldsymbol{u}^i_h}
\newcommand{\tpressh}{q_{h}}
\newcommand{\tpressbh}{q^{b}_h}
\newcommand{\tpresseh}{q^{e}_h}
\newcommand{\tpressih}{q^{i}_h}
\newcommand{\konvh}{\boldsymbol{c}^{e}_h} % konvective velocity
\newcommand{\bodyfh}{\boldsymbol{b}^f_h}

%test functions
\newcommand{\tveli}{\boldsymbol{v}^{i}}
\newcommand{\tvelb}{\boldsymbol{v}^{b}}
\newcommand{\tvele}{\boldsymbol{v}^{e}}
\newcommand{\tvel}{\boldsymbol{v}}
\newcommand{\tpressb}{q^{b}}
\newcommand{\tpresse}{q^{e}}
\newcommand{\tpress}{q}

% governing equations variables
\newcommand{\cauchystress}{\boldsymbol{\sigma}} %cauchy
\newcommand{\cauchystressb}{\boldsymbol{\sigma}^{b}}
\newcommand{\cauchystresse}{\boldsymbol{\sigma}^{e}}
\newcommand{\shearstress}{\boldsymbol{\tau}} %shear stress
\newcommand{\bodyf}{\boldsymbol{b}^{\text{f}}}
\newcommand{\idendity}{\boldsymbol{I}}
\newcommand{\visc}[1]{\boldsymbol{\epsilon}(#1)}

% stress-based
\newcommand{\cauchybar}{{\overline{\boldsymbol\sigma}^b}}
\newcommand{\cauchybarh}{{\overline{\boldsymbol\sigma}^b_h}}
\newcommand{\tcauchybar}{{\overline{\boldsymbol\tau}^b}} %cauchybar
\newcommand{\tcauchybarh}{{\overline{\boldsymbol\tau}^b_h}} %cauchybar

% mathematical operators (jumps, averages, Div, Grad ...)

\newcommand{\Div}{\nabla\cdot}																% divergence operator
\newcommand{\Grad}{\nabla}
\newcommand{\scalL}[3]{\big(#1,#2 \big)_{{\Omega}^{#3}}} %L2-Skalarprodukt
\newcommand{\scalLtime}[3]{\big(#1,#2 \big)_{{\Omega}^{#3}(t^{n+1})}} %L2-Skalarprodukt
\newcommand{\scalintL}[2]{\left<#1,#2 \right>_{\interfaceff}} %L2-Skalarprodukt
\newcommand{\scalintLgeneral}[3]{\left<#1,#2 \right>_{#3}} %L2-Skalarprodukt
\newcommand{\scalintLgeneralnp}[3]{\left<#1,#2 \right>_{#3(t^{n+1})}} %L2-Skalarprodukt
\newcommand{\scalintLnp}[2]{\left<#1,#2 \right>_{\interfaceffnp}} %L2-Skalarprodukt
\newcommand{\scalintN}[2]{\left<#1,#2 \right>_{\partial \domainbf_N}} %neumann
\newcommand{\scalintNgeneral}[2]{\left<#1,#2 \right>_{\partial \domainf_N}} %neumann
\newcommand{\scalintNgeneralnp}[2]{\left<#1,#2 \right>_{\partial \domainf_N(t^{n+1})}} %neumann
\newcommand{\scalintNtime}[2]{\left<#1,#2 \right>_{\partial \domainbf_N(t^{n+1})}} %neumann
\newcommand{\scalintD}[2]{\left<#1,#2 \right>_{\domainbf_D}} %Dirchlet
\newcommand{\scalintNs}[2]{\left<#1,#2 \right>_{\partial \domains_N}} %neumann str

\newcommand{\norm}[2]{\|#1\|_{L^2(#2)}} %L^2-Norm auf 

%jumps, averge..
\newcommand{\jump}[1]{\ensuremath{[\![#1]\!]} }
\newcommand{\averg}[1]{\ensuremath{\{#1\}} }
\newcommand{\avergtwo}[1]{\ensuremath{\langle#1\rangle} }

\DeclareMathOperator{\dx}{dx}
\DeclareMathOperator{\ds}{ds}
\DeclareMathOperator{\domega}{d \Omega}
%---------------------------------------------------------------------------------------------
